Similar in vivo killing efficacy of polyoma virus-specific CD8 T cells during acute and chronic phases of the infection

Viral infections can be broadly divided into infections that are cleared from the host (acute) and those that persist (chronic). Why some viruses establish chronic infections while other do not is poorly understood. One possibility is that the host's immune response is impaired during chronic infections and is unable to clear the virus from the host. In this report we use a recently proposed framework to estimate the per capita killing efficacy of CD8$^+$ T cells, specific for the MT389 epitope of polyoma virus (PyV), which establishes a chronic infection in mice. Surprisingly, the estimated per cell killing efficacy of MT389-specific effector CD8$^+$ T cells during the acute phase of the infection was very similar to the previously estimated efficacy of effector CD8$^+$ T cells specific to lymphocytic choriomeningitis virus (LCMV-Armstrong), which is cleared from the host. We also find that during the chronic phase of the infection the killing efficacy of PyV-specific CD8$^+$ T cells was only half of that of cells in the acute phase. This decrease in the killing efficacy is again surprisingly similar to the change in the killing efficacy of LCMV-specific CD8$^+$ T cells from the peak of the response to the memory phase. Interestingly, we also find that PyV-specific CD8$^+$ T cells in the chronic phase of the infection require lower doses of antigen to kill a target cell. In summary, we find little support for the hypothesis that persistence of infections is caused by inability of the host to mount an efficient immune response, and that even in the presence of an efficient CD8$^+$ T cell response, some viruses can still establish a persistent infection.

==> papersize.tex <==
\advance\voffset by -1cm \advance\hoffset by -1.2cm
\textheight=21cm \textwidth=17cm
%\advance\voffset by -0.6in \advance\hoffset by -0.5in
%\textheight=9in \textwidth=6.3in
\parskip 0.4cm

